Auto-Cypher: Improving LLMs on Cypher generation via LLM-supervised generation-verification framework

Graph databases like Neo4j are gaining popularity for handling complex, interconnected data, over traditional relational databases in modeling and querying relationships. While translating natural language into SQL queries is well-researched, generating Cypher queries for Neo4j remains relatively underexplored. In this work, we present an automated, LLM-Supervised, pipeline to generate high-quality synthetic data for Text2Cypher. Our Cypher data generation pipeline introduces LLM-As-Database-Filler, a novel strategy for ensuring Cypher query correctness, thus resulting in high quality generations. Using our pipeline, we generate high quality Text2Cypher data - SynthCypher containing 29.8k instances across various domains and queries with varying complexities. Training open-source LLMs like LLaMa-3.1-8B, Mistral-7B, and QWEN-7B on SynthCypher results in performance gains of up to 40% on the Text2Cypher test split and 30% on the SPIDER benchmark, adapted for graph databases.

==> latex/1Introduction.tex <==
\section{Introduction}




\paragraph{}Graph databases such as Neo4J Cypher \cite{neo4j} are becoming an increasingly popular alternative to their relational counterparts such as SQL as they avoid rigid tables and provide a more natural and interpretable data representation. While solutions like Text2SQL for relational databases have been extensively studied \cite{Deng_2021} \cite{yu-etal-2018-spider}, \cite{li2023llmservedatabaseinterface} \cite{shi2024surveyemployinglargelanguage} their counterparts for graph databases (Text2Cypher) are still emerging. Cypher \cite{francis2018cypher} is a popular query language for Neo4j knowledge graph databases and is an important interface for graph analytics, with hundreds of thousands of users worldwide. 

We observed that popular open-source models fall short of expected performance on the Text2Cypher task.  Furthermore, these models are limited by a lack of good datasets to fine tune. Thus, existing methods for natural language to Cypher query generation are often too limited or domain-specific, making automation inefficient. To address these gaps, we introduce a synthetic dataset and pipeline designed to train LLMs in generating Cypher queries from natural language inputs. We construct a large training corpus and a test benchmark using this our proposed pipeline. Our dataset covers a wide range of query types, domains, and schemas, helping LLMs better translate user intents into executable Cypher queries.

% A pertinent question to ask here is: how does Cypher specifically help relational style table? The answer is that one can abstract out the various relationships between relational database tables themselves as a graph data structure with tables acting as nodes, and foreign key relationships acting as edges.

One such application that can benefit from this approach is Virtual Agent, where a chatbot is interacting with a user to fulfill a catalog request through conversation. Often, a catalog item asks for information that can already be answered from an internal database table (such as assets owned (ITSM), home address (HR) etc.). Instead of requesting this from the user, we can retrieve it from existing tables across BUs to deliver a smarter and user-friendly experience. Knowledge graphs also play a crucial role within the Retrieval Augmented Generation (RAG) framework \cite{RAG}\cite{gao2024retrievalaugmentedgenerationlargelanguage} of Large Language Models (LLMs). Yet, current tools do not fully support the seamless translation of natural language into Cypher queries, essential for interacting with graph databases.

Our experiments show that fine-tuning LLMs with our synthetically generated dataset significantly improves their ability to generate accurate Cypher queries. 

==> latex/3Approach.tex <==

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{latex/figures/text2cypher.pdf}
    \caption{Caption}
    \label{fig:pipeline}
\end{figure*}

\section{Approach}

\paragraph{}Synthetic data generation strategies\cite{xu2023wizardlm,luo2023wizardcoder,ouyang2022training,zhou2023lima} have been shown to be an effective way to mimic human generated data, and even surpass it. We rely on the creativity and instruction following ability of the current generation of LLMs such as Llama 3.1 70B\cite{maaten2024llama3}, Mixtral 8*22B\cite{Jiang2024MixtralOE} and GPT-4\cite{openai2023gpt4} to construct the domains, schemas, questions and cypher queries required for our task from scratch. To reduce noisy and incorrect samples, we also build a pipeline for validation of the generated data points to preserve only high confidence samples by executing the generated cypher query and validating the results (see Figure~\ref{fig:complete_pipeline}). We also ensure that we cover a large diversity of domains as well as query types by conditioning the generation on over \textbf{109 query taxonomies} (refer Appendix~\ref{sec:querytypes}). and \textbf{700 domains}.



Diagram from Masoud here. Label/Index the diagram blocks in numbers and discuss each block in the same order. Guide the readers by refering the blocks as if in a walkthrough diagram. \textcolor{red}{Shorten the following subsections.}


\subsection{Domains}We start with a list of seed domains taken from Neo4J\cite{neo4j} example databases, as well as manually curated domains relevant to ServiceNow such as ecommerce, supply chain and inventory management etc. Then we prompt Mixtral\cite{Jiang2024MixtralOE} (\ref{sec:appendixB}) with a higher temperature setting (0.7) to generate additional such domains and dedupe the results obtained over several calls. Cumulatively, this yielded 700 distinct domains

\subsection{Schema Extraction and Validation}For each domain, we generate an example Cypher schema by prompting the model to generate a skeleton schema with nodes and relationships that can be plausible in that domain as shown in Appendix-B. Next, we expand the skeleton schema by adding various synthetic properties to the nodes and relationships, as well as forming edges between the nodes using the relationships(\ref{sec:appendixB}). We augment our generated schemas with a list of real-world test schemas sourced from Neo4J example databases\cite{neo4j}.  We subject the generated schemas to additional layer of GPT-4 scrutiny. Additionally, we manually verified 25\% of the schemas to ensure coherence, usefulness and correctness before proceeding further. These validation steps were critical as the correctness of the schema lays a solid foundation for the synthetic data generation that follows next.

\subsection{Question Generation}For each schema, we randomly select certain number of query types from 109 pre-defined query types synthesized using Mixtral\cite{Jiang2024MixtralOE} to generate corresponding natural language questions (see Figure~\ref{fig:question_generation}). Query types (refer Appendix~\ref{sec:querytypes}) include a wide range of taxonomy such as "Simple Retrieval Queries" "Multi-Criteria Retrieval Queries" or "Complex Aggregation Queries", “Sub-Graph queries” etc. This conditional generation ensures that we cover various facets of Cypher's querying capabilities to create a diverse set of questions that represent a wide range of real-world scenarios.


\subsection{Cypher Query Generation}Next, Mixtral is used to generate the corresponding Cypher query for the natural language question on that schema. The model follows a chain-of-thought reasoning process\cite{wei2022chain}, where the generation happens in multiple stages (\ref{sec:cypher_generation}). This multi-step approach helps ensure that the model can reason through the question and the schema sufficiently before generating the candidate cypher for the further validation steps.

\subsection{Validation of Cypher queries}This section goes over our novel approach to validating the generated cyphers. While llm-as-judge\cite{zheng2023judging} approaches have been widely tried in SQL literature, this approach cannot guarantee that the cypher will execute and return results as expected. To overcome this limitation, we cleverly use the LLM (GPT-4) as database constructor and then execute the cyphers on that database. To the best of our knowledge, this strategy has not been explored in literature before. This happens in three steps:
\subsubsection{Synthetic Ground Truth Generation}For each question, we generate a dummy ground truth, which is of the expected structure, data-type and is plausibly true for that question. For e.g.
\smallskip

\textbf{Question:} What is the total sales in USD for Apples in the California market and who made the most sales?

$\textbf{Dummy answer:} \{``total\_sales\_usd'': 10000, ``employee'': ``John Doe''\}$

\smallskip
Next, we construct a dummy database, filling the data in such a way that the \textit{dummy answer} is the \textbf{right answer} for that question.
\vspace{-5pt}
\subsubsection{Code Generation for Database Population}We prompt GPT-4\cite{openai2023gpt4} to fill a test database per criteria in the above section. In this step, the model generates Python code to populate a Neo4j database with synthetic data. The code generation follows a two-step process (\ref{sec:code_generation}). Firstly to plan and reason with ample detail and then write python code to fill the database with both pertinent (to the question) and other data points.






\subsection{Final validation}The cypher queries are executed against the dummy database and the obtained results are validated against the dummy ground truth generated earlier. If the results match the ground truth, the Cypher query is considered correct and is stored in the dataset. If the query fails to produce the correct result, the process is repeated or refined until a valid query is generated. Note that we only use GPT-4 for validation, so none of it's generated tokens go into the dataset. Additionally, we subject a small sample to manual validation and checked that all the cyphers are correct.

At the end of this process, we have a complete dataset consisting of these rows: \texttt{Schema},  \texttt{Question}, \texttt{Data population queries}, \texttt{Cypher Query} and \texttt{Execution Results}. This dataset can now be used for training or evaluating models tasked with converting natural language queries into Cypher code.





